LayoutRectifier: An Optimization-based Post-processing for Graphic Design Layout Generation

Recent deep learning methods can generate diverse graphic design layouts efficiently. However, these methods often create layouts with flaws, such as misalignment, unwanted overlaps, and unsatisfied containment. To tackle this issue, we propose an optimization-based method called LayoutRectifier, which gracefully rectifies auto-generated graphic design layouts to reduce these flaws while minimizing deviation from the generated layout. The core of our method is a two-stage optimization. First, we utilize grid systems, which professional designers commonly use to organize elements, to mitigate misalignments through discrete search. Second, we introduce a novel box containment function designed to adjust the positions and sizes of the layout elements, preventing unwanted overlapping and promoting desired containment. We evaluate our method on content-agnostic and content-aware layout generation tasks and achieve better-quality layouts that are more suitable for downstream graphic design tasks. Our method complements learning-based layout generation methods and does not require additional training.

==> alg_files/search_and_snap_alg.tex <==
\begin{algorithm}[h]
\caption{Search-and-snap}
\label{alg:sas}
\begin{algorithmic}[1]
\INPUT current layout $L$, a example grid system $G^{e}$, all snap options $S$.
\OUTPUT refined layout $\tilde{L}$.

\For{$(c, b) \in L$}
    \State bestSnapIndex $\gets -1$
    \State bestScore $\gets 10000$
    \For{$s \in S$}
        \State $\bar{b} \gets \text{snap}(b, s)$
        \State $\text{score}(\bar{b}) \gets \mathcal{E}_{\text{all}}(L\setminus b \cup\bar{b})$
        \If{$\text{score}(\bar{b}) < \text{bestScore}$}
            \State $\text{bestScore} \gets \text{score}(\bar{b})$
            \State $\text{bestScoreIndex} \gets s$
        \EndIf
    \EndFor
    \Statex \LeftComment{1}{Update layout set $L$ using the snapped box.}
    \State $L \gets L\setminus b \cup \text{snap}(b,\text{bestSnapIndex})$
% \State $aa$\text
\EndFor
% \State $\mathbf{G}^{e} \gets \text{retrieve}(L, \mathbf{L})$ 
% \State $\mathcal{R} \gets \text{detect-alignment}(L)$
% \State $\mathbf{\hat{L}} \gets \emptyset$
% \For{$G^{e}_{k} \in \mathbf{G}^{e}$}
%     \Statex \LeftComment{1}{$T$: max iteration number}
%     \For{$t \gets 1$ to $T$} 
%         \State $L_t \gets \text{search-and-snap}(L_t, G^{e}_{k}, \mathcal{R})$
%         \Statex \LeftComment{2}{$L_t$: refined layouts after at $t$-th iteration}
%         \State $L_t \gets \text{minimize } (\mathcal{L}_{\text{overlay}}(L_t) +  \mathcal{L}_{\text{underlay}}(L_t)$) 
%     \EndFor
%     % \State $\bar{L} \gets \bar{L}_t$
% \If{valid($L_{T}$)}
%     \State $\mathbf{\hat{L}} \gets \mathbf{\hat{L}} \cup \{L_{T}\}$
% \EndIf
% \EndFor
% \State \textbf{return} $\mathbf{\hat{L}}$
% \State $\hat{\theta}_j=(\hat{\mathcal{A}}_j,\hat{\mathcal{D}}_j) \gets \text{WarpNet}((I_j, I_T))$ \Comment{\Cref{sec:warpnet}}
% \State $\hat{G}_j \gets \mathcal{T}_{\hat{\theta}_j}(G_j)$ \Comment{TPS transformation}
% \State $S_{j+1} \gets \text{Warp}(S_{j},\hat{G}_j)$    
% \State \Return $S_{j+1}$
\end{algorithmic}
\end{algorithm}

==> cgf/cgf_metadata.tex <==
\title[\methodName: An Optimization-based Post-processing for Graphic Design Layout Generation]%
      {\methodName: An Optimization-based Post-processing for Graphic Design Layout Generation}

\author[paper1002]{paper1002}

\author[I-Chao Shen et al.]
{\parbox{\textwidth}{\centering I-Chao Shen$^{1}$\orcid{0000-0003-4201-3793} ~ Ariel Shamir$^{2}$\orcid{0000-0001-7082-7845} ~ Takeo Igarashi$^{1}$\orcid{0000-0002-5495-6441}
%        S. Spencer$^2$\thanks{Chairman Siggraph Publications Board}
        }
        \\
% For Computer Graphics Forum: Please use the abbreviation of your first name.
{\parbox{\textwidth}{\centering $^1$ The University of Tokyo, Japan \\
$^2$ Reichman University, Israel
%        $^2$ Another Department to illustrate the use in papers from authors
%             with different affiliations
      }
}
}

% add teaser here.
\input{fig_files/teaser_fig}


==> fig_files/ablation_size_preserve_fig.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{figs/ablation_size_v0.pdf}
  \caption{
  \textbf{Ablation study on the preservation terms.}
 We compared the refined layouts generated with and without the size and aspect ratio preservation terms. 
    The size and aspect ratio of elements are better preserved with the preservation terms. 
  }
  \label{fig:ablation_size}
\end{figure}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figs/prompt_comp.pdf}
%   \caption{
%   \todo{To be removed.}
%   Comparison between the refined layouts generated by our method and LayoutPrompter~\cite{lin2024layoutprompter} using the same set of examples.
%   For PubLayNet layout, our results improve alignments and avoid overlapping while the results of LayoutPrompter still contain undesired overlappings.
%   For Magazine layout, LayoutPrompter fails to generate layout contains desired underlay.
%   % (``text-over-image'' elements are not contained by ``image'' elements).
%   }
%   \label{fig:prompt_comp}
% \end{figure}



==> fig_files/align_detection_fig.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figs/align_detect.pdf}
  \caption{
  % \todo{Update this figure small caption -> remove detect..}
  The criteria we used to detect (a) vertical and (b) horizontal alignments.}
  \label{fig:align_detection}
\end{figure}

==> fig_files/align_type_fig.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figs/align_type.pdf}
  \caption{We extract eight different alignment categories between pair of element boxes.}
  \label{fig:align_type}
\end{figure}

==> fig_files/limitation_minkos_fig.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/minkowski_compare.pdf}
  \caption{
  \textbf{Minkowski penalty comparison.}
  Given the (a) input layout, Minkowski penalty successfully mitigate unwanted overlaps (b) with and (c) without using a reference grid but cannot resolve the misalignment. Moreover, it fails to preserve the similarity to the input layout.
  }
  \label{fig:minkowski}
\end{figure}

==> fig_files/magazine_improve_discuss_fig.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/magazine_improvement.pdf}
  \caption{
  \todo{discuss the improvement differneces.}
  The improvement of each metric of the Magazine dataset.
  }
  \label{fig:align_detection}
\end{figure}

==> fig_files/minkowski_comparison_fig.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/minkowski_compare.pdf}
  \caption{\textbf{Minkowski penalty comparison.}
  % \todo{For the failure case, maybe we need to find a more extreme case?}
  % \todo{Check can we do the weight changes to }
  }
  \label{fig:limitation}
\end{figure}

%% publaynet: blt-800

==> fig_files/prompter_comp_fig.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figs/prompt_comp_v2.pdf}
  \caption{
% \todo{Maybe move to supp material.}
\todo{Revise the caption.}
  \textbf{Qualitative comparison with LayoutPrompter~\cite{lin2024layoutprompter}.} 
  % We compared the refined layouts generated by our method and CLG~\cite{kikuchi2021constrained} for (a) PubLayNet and (b) Magazine datasets.
  % The refined layouts generated by our method improves have better alignment and overlay compared to the results generated by CLG.
  % Meanwhile, CLG cannot keep the underlay relationship (``text-over-image'' in the ``image'') that the original input layout has.
  % Meanwhile, the layouts refined by CLG ail to preserve the structure and relations between elements in the input layout.
  % (\protect \blackline represents elements with undesired overlaps.)
  }
  % publaynet: layoutganpp-1 (up) -> keep
  % publaynet: layoutganpp-6 (bottom)
  % magazine layoutganpp-6 for no containment
  % magazine 11 for changing the layout too much -> keep
  \label{fig:prompter_comp_qual}
\end{figure}

==> fig_files/publaynet_stat_fig.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{figs/stat_publaynet.pdf}
  \caption{\todo{Maybe remove?}The overlay and alignment distributions of publaynet dataset.}
  \label{fig:publaynet_stat}
\end{figure}

==> fig_files/sas_example_fig.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.9\linewidth]{figs/sas_example.pdf}
  \caption{
  (a) Element box $b_i$ can snap by vertex or edge.
  (b,c) In both vertex snap options, $b_i$ causes undesired overlaps.
  (d,e) In both edge snap options, $b_i$ results in undesired overlaps and misalignments.
  (f) Our method selects the best snap option that avoids both overlap and misalignment.
  (orange point and line indicate snap vertex and edge.)
  }
  \label{fig:sas_example}
\end{figure}

==> fig_files/size_ablation_supp_fig.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figs/size_ablation_supp.pdf}
  \caption{
% \todo{Check the figure carefully there is a wrong figure..}
  \textbf{Qualitative comparison of element preserving ablation study.} We compared the refined layouts generated with and without the size and aspect ratio preservation terms. 
    The size and aspect ratio of elements are better preserved in the layouts generated with the preservation terms. 
  }
  \label{fig:supp_size_ablation}
\end{figure}

==> fig_files/snap_options_fig.tex <==
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figs/snap_options_all.pdf}
  \caption{Our method allows both (a) edge snap and (b) vertex snap.
  (a) In edge snap, the highlighted edge of the element box will snap to the highlighted edge of the grid.
  (b) Similarly, in vertex snap, the highlighted vertex of the element box will snap to the highlighted vertex of the grid.
  }
  \label{fig:snap_options}
\end{figure}

==> fig_files/user_study_ui_fig.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{figs/user_study_ui.png}
  \caption{
    \textbf{User interface of our user study.}
  }
  \label{fig:user_study_ui}
\end{figure}

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{figs/prompt_comp.pdf}
%   \caption{
%   \todo{To be removed.}
%   Comparison between the refined layouts generated by our method and LayoutPrompter~\cite{lin2024layoutprompter} using the same set of examples.
%   For PubLayNet layout, our results improve alignments and avoid overlapping while the results of LayoutPrompter still contain undesired overlappings.
%   For Magazine layout, LayoutPrompter fails to generate layout contains desired underlay.
%   % (``text-over-image'' elements are not contained by ``image'' elements).
%   }
%   \label{fig:prompt_comp}
% \end{figure}



==> latexmkrc <==
# --- This file allows you to quickly change the style in case you need to resubmit
$ENV{'TEXINPUTS'}='./cvpr//:./eccv//:./cgf//:./iccv//:' . $ENV{'TEXINPUTS'}; 
$ENV{'BSTINPUTS'}='./cvpr//:./eccv//:./cgf//:./iccv//:' . $ENV{'BSTINPUTS'};

$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> overview.tex <==
\section{Overview}

==> prob_formulation.tex <==
\subsection{Problem Formulation}
%% talk about how we treat each document.
In this paper, each layout $L$ consists of a set of layout elements $L=[l_0, l_1, ..., l_N]$, where $N$ is the number of elements in $L$.
Each element $l_i$ is described using five attributes, \ie~$(c, w, h, x, y)$,  in which the first element $c\in C$ is the object category such as the logo or button, and the remainder details the bounding box information, \ie~the center location $(x, y)\in \mathcal{R}^2$ and the width and height $(w, h)\in \mathcal{R}^2$.


In this paper, we focus on conditional layout generation, \ie~the input of our method is the number of elements and element types.
Following previous works~\cite{kong2022blt}, we describe each layout element using five attributes, \ie~$(c, w, h, x, y)$,  in which the first element $c\in C$ is the object category such as the logo or button, and the remainder details the bounding box information, \ie~the center location $(x, y)\in \mathcal{R}^2$ and the width and height $(w, h)\in \mathcal{R}^2$.
Furthermore, float values in bounding box information is discretized using $8$-bit uniform quantization.
A layout $L$ of $K$ assets is hence denoted as a flattened sequence of integer indices:
\begin{align}
L = [\langle\text{bos}\rangle, c_1, w_1, h_1, x_1, y_1, ..., c_K, w_K, h_K, x_K, y_K, \langle\text{eos}\rangle]
\end{align}





==> tab_files/ablation_quan_result.tex <==
\begin{table*}[!h]
\small
\centering
\begin{adjustbox}{width=1.0\linewidth, center}
\subfloat[PubLayNet]{\label{tab:tab1a}{
\begin{tabular}{c|ccc|ccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Ove$\downarrow$}} & \multicolumn{3}{c}{\textbf{Align (x100)$\downarrow$}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
\backslashbox{Gen}{Refine} & {Ori} & {\sighl{w/o Stage A}} &{Ours} & {Ori} & {\sighl{w/o stage A}} & {Ours} \\
\midrule
% Autoreg & 0.22 & ? & 0.015 & ? & 0.124 & ? & 0.89 & ?\\
LGAN++&  0.108& 0.021 &\bestcell{0.0016} & 0.18 & 0.036 & \bestcell{0.031}\\
BLT&  1.049& 0.423 &\bestcell{0.18} & 0.139 & 0.083 & \bestcell{0.061} \\
LDM&  0.155 & 0.048 &\bestcell{0.006} & 0.12 & 0.043 & \bestcell{0.025} \\
LF++&  0.009 & \bestcell{0.003} &\bestcell{0.003} & 0.023 & 0.003 & \bestcell{0.002}\\
\bottomrule
\end{tabular}
}
}
\subfloat[Magazine]{\label{tab:tab1b}{
\begin{tabular}{c|ccc|ccc|ccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Ove$\downarrow$}} & \multicolumn{3}{c}{\textbf{Align (x100)$\downarrow$}} &\multicolumn{3}{c}{\textbf{Cont$\uparrow$}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
\backslashbox{Gen}{Refine} & {Ori} & {\sighl{w/o stage A}} &{Ours} & {Ori} & {\sighl{w/o stage A}} & {Ours} & {Ori} & {\sighl{w/o stage A}} & {Ours} \\
\midrule
% Autoreg & 0.22 & ? & 0.015 & ? & 0.124 & ? & 0.89 & ?\\
LGAN++&  0.387& 0.253 &\bestcell{0.204} & 0.924 & 0.717 & \bestcell{0.273} & 0.409 & 0.424 & \bestcell{0.455}\\
BLT&  0.739 & 0.466 & \bestcell{0.353} & 0.601 & 0.389 & \bestcell{0.305} & 0.269 & 0.284 & \bestcell{0.375} \\
LDM&  0.633 & 0.411 &\bestcell{0.213} & 0.468 & 0.848 & \bestcell{0.269} & 0.307 & 0.328 & \bestcell{0.404} \\
LF++&  0.742 & 0.360 &\bestcell{0.219} & 0.467 & 0.715 & \bestcell{0.269} & 0.371 & 0.108 & \bestcell{0.282}\\
\bottomrule
\end{tabular}
}
}
\end{adjustbox}
\caption{
% \todo{Maybe move this to supp...}
\textbf{Quantitative result of ablation study on stage A.}
}
\label{tab:ablation_quan}
\end{table*}

==> tab_files/ablation_stage_B_quan_result.tex <==
\begin{table*}[!h]
\small
\centering
\begin{adjustbox}{width=1.0\linewidth, center}
\subfloat[PubLayNet]{\label{tab:tab1a}{
\begin{tabular}{c|ccc|ccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Ove$\downarrow$}} & \multicolumn{3}{c}{\textbf{Align (x100)$\downarrow$}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} 
\backslashbox{Gen}{Refine} & {Ori} & {\sighl{w/o Stage B}} &{Ours} & {Ori} & {\sighl{w/o stage B}} & {Ours} \\
\midrule
LGAN++&  0.108 & 0.14 &\bestcell{0.0016} & 0.18 & \bestcell{0.025} & 0.031\\
BLT&  1.049& 1.03 &\bestcell{0.18} & 0.139 & \bestcell{0.057} & 0.061 \\
LDM&  0.155 & 0.136 &\bestcell{0.006} & 0.12 & \bestcell{0.023} & 0.025 \\
LF++&  0.009 & 0.006 &\bestcell{0.003} & 0.023 & \bestcell{0.002} & \bestcell{0.002}\\
\bottomrule
\end{tabular}
}
}
\subfloat[Magazine]{\label{tab:tab1b}{
\begin{tabular}{c|ccc|ccc|ccc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Ove$\downarrow$}} & \multicolumn{3}{c}{\textbf{Align (x100)$\downarrow$}} &\multicolumn{3}{c}{\textbf{Cont$\uparrow$}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
\backslashbox{Gen}{Refine} & {Ori} & {\sighl{w/o stage B}} &{Ours} & {Ori} & {\sighl{w/o stage B}} & {Ours} & {Ori} & {\sighl{w/o stage B}} & {Ours} \\
\midrule
% Autoreg & 0.22 & ? & 0.015 & ? & 0.124 & ? & 0.89 & ?\\
LGAN++&  0.387& 0.371 &\bestcell{0.204} & 0.924 & \bestcell{0.263}& 0.273 & 0.409 & 0.418 & \bestcell{0.455}\\
BLT&  0.739 & 0.698 & \bestcell{0.353} & 0.601 & \bestcell{0.287} & 0.305 & 0.269 & 0.294 & \bestcell{0.375} \\
LDM&  0.633 & 0.646 &\bestcell{0.213} & 0.468 & 0.277 & \bestcell{0.269} & 0.307 & 0.331 & \bestcell{0.404} \\
LF++&  0.742 & 0.587 &\bestcell{0.219} & 0.467 & \bestcell{0.231} & 0.269 & 0.371 & 0.149 & \bestcell{0.282}\\
\bottomrule
\end{tabular}
}
}
\end{adjustbox}
\caption{
% \todo{check magazine numbers..}
% \todo{Make this smaller.}
% \todo{Maybe move this to supp...}
\textbf{Quantitative result of ablation study on stage B.}
}
\label{tab:ablation_quan_B}
\end{table*}

==> tab_files/test_table.tex <==
\begin{table}[]
\caption{
Quantitative result of the ablation study on the regularization for the latent space.
}
\begin{tabular}{llcccc}
\toprule
&  & 
\begin{tabular}[c]{@{}c@{}}Task 1\\ ($D_{\text{voxel}} $)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Task 2\\ ($D_{\text{chamfer}}$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Task 3\\ ($D_{\text{chamfer}}$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Task 4\\ ($D_{\text{chamfer}}$)\end{tabular} \\
\midrule
\midrule
\multirow{2}{*}{Table}& Ours         & \bestcell{0.5417}                                      & \bestcell{0.0002}                                       & \bestcell{0.0006}                                       & \bestcell{0.0030}                                       \\
 & w/o Reg          & 0.6900                                               & 0.0011                                                & 0.0046                                                & 0.0232                                                \\
\midrule
\multirow{2}{*}{Sofa}  & Ours         & \bestcell{0.4998}                                      & \bestcell{0.0007}                                       & \bestcell{0.0009}                                       & \bestcell{0.0071}                                  \\
& w/o Reg         & 0.8300                                               & 0.0026                                                & 0.0087                                                & 0.0050                                                \\
\midrule
\multirow{2}{*}{Chair}& Ours         & \bestcell{0.4006}                                      & \bestcell{0.0004}                                       & 0.0032                                                & \bestcell{0.0144}                                       \\
 &  w/o Reg          & 0.5200                                               & 0.0006                                                & \bestcell{0.0028}                                       & 0.0147                                                \\
\midrule
\multirow{2}{*}{Shelf} & Ours         & \bestcell{0.9408}                                      & \bestcell{0.0008}                                       & \bestcell{0.0063}                                       & \bestcell{0.0090}                                       \\
 &  w/o Reg          & 1.0580                                               & 0.0010                                                & 0.0327                                                & 0.0440                                                \\
\midrule
\multirow{2}{*}{Bed}   & Ours         & 0.1182                                               & 0.0004                                                & \bestcell{0.0009}                                       & 0.0073                                                \\
& w/o Reg          & \bestcell{0.0070}                                      & \bestcell{0.0003}                                       & 0.0053                                                & \bestcell{0.0054}                                       \\
\bottomrule
\end{tabular}
\label{tab_ablation}
\end{table}

==> tab_files/training_free_quan_result.tex <==
\begin{table*}[h]
\small
\centering
\subfloat[PubLayNet]
{\label{tab:free_pub}{
\begin{tabular}{c|ccc|ccc|cc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Ove $\downarrow$}} & \multicolumn{3}{c}{\textbf{Align (x100) $\downarrow$}} & \multicolumn{2}{c}{\sighl{\textbf{Sim $\uparrow$}}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-9}
\textbf{ori method} & {Ori} & LP & {Ours} & {Ori} & LP & {Ours} & LP & {Ours}\\
\midrule
LGAN++  & 0.108 & 0.018 &\bestcell{0.0016} & 0.18 & \seccell{0.176} & \bestcell{0.031} & 0.648 & \bestcell{2.616} \\
BLT  & 1.049  & \seccell{0.40} &\bestcell{0.18} & \seccell{0.139}  & 0.645 &  \bestcell{0.061} & 0.417 & \bestcell{2.05} \\
LDM & 0.155 & \seccell{0.146} &\bestcell{0.006} & 0.12  & \bestcell{0.021} &\seccell{0.025}  & 0.357 & \bestcell{2.507}\\
LF++ & 0.009 & ? &\bestcell{0.003} & 0.44 & ? & \bestcell{0.0015} & ?& \bestcell{2.866} \\
% LayoutPrompter & 0.037 & ? & 0.047 & ? \\
\bottomrule
\end{tabular}
}
}\\
\subfloat[Magazine]
{\label{tab:free_mag}{
\begin{tabular}{c|ccc|ccc|ccc|cc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Ove $\downarrow$}} & \multicolumn{3}{c}{\textbf{Align (x100) $\downarrow$}} & \multicolumn{3}{c}{\textbf{Cont $\uparrow$}} & \multicolumn{2}{c}{\textbf{Sim $\uparrow$}}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12}
\textbf{ori method} & {Ori} & LP & {Ours} & {Ori} & LP & {Ours} & {Ori} & LP & {Ours} & LP & {Ours}\\
\midrule
LGAN++ & 0.387 &  \seccell{0.360} &\bestcell{0.204} & 0.924 &  \seccell{0.281} & \bestcell{0.273}& 0.409 &  \seccell{0.413} &\bestcell{0.455} & 0.477 & \bestcell{1.828} \\
BLT  & 0.739 & \seccell{0.392} & \bestcell{0.353} & 0.742 & \seccell{0.645} &\bestcell{0.305} & \seccell{0.269} & 0.342 & \bestcell{0.375} & 0.551 & \bestcell{1.051}\\
LDM  & 0.633 &  \seccell{0.415} & \bestcell{0.213} & 1.01 & \seccell{0.563} & \bestcell{0.388} &  \seccell{0.309} & 0.371 &\bestcell{0.404} & 0.837 & \bestcell{1.483}\\
LF++ & 0.742 &  \seccell{0.394} &\bestcell{0.219} & \seccell{0.467} &   0.607 &\bestcell{0.269}  & \bestcell{0.370} &  0.273 & \seccell{0.282} & 0.287 & \bestcell{0.794}\\
\bottomrule
\end{tabular}
}
}
\caption{
% \todo{Check similarity...}
\textbf{Training-free method comparison of PubLayNet and Magazine dataset.}
}
\label{tab:training_free_quan}
\end{table*}
